Automated analysis of security protocols with global state

Security APIs, key servers and protocols that need to keep the status of transactions, require to maintain a global, non-monotonic state, e.g., in the form of a database or register. However, most existing automated verification tools do not support the analysis of such stateful security protocols - sometimes because of fundamental reasons, such as the encoding of the protocol as Horn clauses, which are inherently monotonic. A notable exception is the recent tamarin prover which allows specifying protocols as multiset rewrite (msr) rules, a formalism expressive enough to encode state. As multiset rewriting is a "low-level" specification language with no direct support for concurrent message passing, encoding protocols correctly is a difficult and error-prone process. We propose a process calculus which is a variant of the applied pi calculus with constructs for manipulation of a global state by processes running in parallel. We show that this language can be translated to msr rules whilst preserving all security properties expressible in a dedicated first-order logic for security properties. The translation has been implemented in a prototype tool which uses the tamarin prover as a backend. We apply the tool to several case studies among which a simplified fragment of PKCS\#11, the Yubikey security token, and an optimistic contract signing protocol.

==> sapic.tex <==
FLATEX  1.21, 1994, 1996, by Sariel Har-Peled.

input file: [translation.tex]

	File: "translation.flt" generated


==> studies-long.tex <==
\begin{figure*}[ht] % (fold)
\centering
\begin{tabular}{c | c c }
Example                                                      & Typing Lemmas & Automated Run\\
\hline
Security API \`a la PKCS\#11                                 & 1             & yes \\
% Needham-Schroeder-Lowe (w/ AS, w/ tagging)                 & not working   & - \\
Yubikey Protocol~\cite{KS-stm12,yubikey}                     & 3             & no\\
GJM Contract-Signing protocol~\cite{ARR-csf11,GJM99}         & 0             & yes\\
Mödersheim's Example (locks/inserts)~\cite{Modersheim-ccs10} & 0             & little interaction \\
Mödersheim's Example (embedded MSRs)~\cite{Modersheim-ccs10} & 0             & yes \\
Security Device Example~\cite{ARR-csf11}                     & 1             & yes\\
Needham-Schroeder-Lowe~\cite{Lowe1996}                       & 1             & yes \\
\end{tabular}
\caption{Case studies.}
\label{fig:case-studies}
% figure case-studies (end)
\end{figure*}

\section{Case studies}
\label{sec:casestudies}

In this section we briefly overview some of the case studies we
performed.  These case studies include a simple security API similar
to PKCS\#11~\cite{PKCS11}, the Yubikey security token, the optimistic
contract signing protocol by Garay, Jakobsson and MacKenzie
(GJM)~\cite{GJM99} and a few other examples, discussed in Arapinis et
al.~\cite{ARR-csf11} and M\"odersheim~\cite{Modersheim-ccs10}. The
results are summarized in \autoref{fig:case-studies}. For each of the
case studies we provide the number of typing lemmas that were needed
by the tamarin prover and whether manual guidance of the tool was
required.  Because of space constraints we do not detail the formal
models of the protocols and properties that we studied. All files of
our prototype implementation and our case studies are available at
\url{\downloadlink}.

\subsection{Security API  \`a la PKCS\#11}

This example illustrates how our modelling might be useful for the
analysis of Security APIs in the style of the PKCS\#11
standard~\cite{PKCS11}.  We expect that studying a complete model of
PKCS\#11, such as in~\cite{DKS-jcs09}, to be a straightforward
extension.  In addition to the processes presented in the running
example in \autoref{sec:calculus} the actual case study models the
following two operations:
\begin{inparaenum}[\it (i)]
\item \emph{encryption:} given a handle and a plain-text, the user can
  request an encryption under the key the handle points to.
\begin{lstlisting}
$P_\mathit{enc}:=$ in(<h,m>); lookup <`att',h> as a in 
       if a=`dec' then lookup <`key',h> as k in
              out(senc(m,k))
\end{lstlisting}
\item \emph{unwrap} given a ciphertext $\mathit{senc}(k_2,k_1)$, and a
  handle $h_1$, the user can request the ciphertext to be
  \emph{unwrapped}, i.e.  decrypted, under the key pointed to by
  $h_1$. If decryption is successful the result is stored on the
  device, and a handle pointing to $k_2$ is returned.
\end{inparaenum}
Moreover, contrary to the running example, at creation time keys are
assigned the attribute `init', from which they can move to either
`wrap', or `unwrap', see the following snippet:
\begin{lstlisting}[numbers=left]
in(<`set_dec',h>); lock <`att',h>;
	 lookup <`att',h> as a in
		if a=`init'	then 
			insert <`att',h>,`dec'; unlock <`att',h>
\end{lstlisting}
Note that, in contrast to the running example, it is necessary to
encapsulate the state changes between lock and unlock. Otherwise an
adversary can stop the execution after line 3, set the attribute to
`wrap' in a concurrent process and produce a wrapping, that he can
decrypt, after resuming operation at line 4, and therefore learn a
key. Such subtleties can produce attacks that our modeling allows to
detect. If locking is handled correctly, we show secrecy of keys
produced on the device, proving the property introduced in
\autoref{ex:property}. If locks are removed the attack described
before is found.


% \subsection{Needham-Schoeder-Lowe}

% We can show secrecy for a session-key established between two honest parties
% running the Needham-Schroeder-Lowe protocol \ref{missing-ref}. The
% modelling does not require tags on the messages.

\subsection{Yubikey}
The Yubikey~\cite{yubikey} is a small hardware device designed to
authenticate a user against network-based services. When the user
presses a button on the device, it outputs a one-time-password
consisting of a counter, a timestamp and other data encrypted using a
key that is on the device. This one-time-password can be used to
authenticate against a server that shares the same secret key.

Among other properties, we show by the means of an injective
correspondence property that an attacker that controls the network
cannot perform replay attacks. A similar analysis has already been
performed by Künnemann and Steel, using tamarin's multiset rewriting
calculus~\cite{KS-stm12}.  However, our model benefits from the more
fine-grained modelling using our new calculus: security-relevant
operations like modeling and tests on state have to be written out in
detail, resulting in a model that is closer to the real-life operation
of such a device. (The modeling of the Yubikey takes approximately 38
lines in our calculus, which translates to 49 multiset rewrite
rules. The modelling by Künnemann and Steel contains only four rules,
but they are are quite complicated, resulting in 23 lines of code.
More importantly, the gap between their model and the actual Yubikey
protocol is larger -- in our calculus, it becomes clear that the
server can treat multiple authentication requests in parallel, as long
as they do not claim to stem from the same Yubikey.)

% it is difficult to ``see'' whether their model is
% faithful with respect to the protocol .)

% \subsection{The GJM contract signing protocol~\cite{GJM99}}
% A contract signing protocol allows two parties to sign a contract in a
% fair way: none of the participants should be bound to the contract
% without the other participant being bound as well. A straightforward
% solution is to use a trusted party that collects both signatures on
% the contract and then sends the signed contracts to each of the
% participants. Optimistic protocols have been designed to avoid the use
% of a trusted party whenever possible (optimizing efficiency, and
% avoiding the potential cost of a trusted party). In these protocols
% the parties first try to simply exchange the signed contracts; in case
% of failure, or cheating behavior of one of the parties, the trusted
% party can be contacted. Depending on the situation, the trusted party
% may either \emph{abort} the contract, or \emph{resolve} it. In case of
% an abort decision the protocol ensures that none of the parties
% obtains a signed contract, while in case of a resolve the protocol
% ensures that both participants obtain the signed contract. For this
% the trusted party needs to maintain a database with the current status
% of all contracts (aborted, resolved, or no decision has been taken).
% In our calculus the status information is naturally modelled using our
% insert and lookup constructs. The use of locks is also crucial here to
% avoid the status to be changed between a lookup and an insert.

% This protocol was also studied by Arapinis et
% al.~\cite{ARR-csf11}. They showed the crucial property that a same
% contract can never be both aborted and resolved. However, due to the
% fact that StatVerif only allows for a finite number of memory cells,
% they have shown this property for a single contract and provide a
% manual proof to lift the result to an unbounded number of
% contracts. We directly prove this property for an unbounded number of
% contracts.


\subsection{Further Case Studies}

We also investigated the case study presented by
Mödersheim~\cite{Modersheim-ccs10}, a key-server example. We encoded
two models of this example, one using the insert construct, the other
manipulating state using the embedded multiset rewrite rules. For
this example the second model turned out to be more natural and more
convenient allowing for a direct automated proof without any
additional typing lemma.

We furthermore modeled the contract signing protocol by Garay et
al.~\cite{GJM99} and a simple security device which both served as
examples in~\cite{ARR-csf11}. In the contract signing protocol a
trusted party needs to maintain a database with the current status of
all contracts (aborted, resolved, or no decision has been taken).  In
our calculus the status information is naturally modelled using our
insert and lookup constructs. The use of locks is indispensable to
avoid the status to be changed between a lookup and an insert.
Arapinis et al.~\cite{ARR-csf11} showed the crucial property that a
same contract can never be both aborted and resolved. However, due to
the fact that StatVerif only allows for a finite number of memory
cells, they have shown this property for a single contract and provide
a manual proof to lift the result to an unbounded number of
contracts. We directly prove this property for an unbounded number of
contracts.
%
% : the device is initialized once to left or
% right. Later on it accepts pairs of encryptions and decrypts either
% the left component of the pair or the right component, but not
% both. As the input language of StatVerif is very similar to ours their
% model could be easily adapted to our tool.
%
Finally we also illustrate the tool's ability to analyze classical
security protocols, by analyzing the Needham Schroeder Lowe
protocol~\cite{Lowe1996}.


